Hacking in the Blind: (Almost) Invisible Runtime UI Attacks on Safety-Critical Terminals

Many terminals are used in safety-critical operations in which humans, through terminal user interfaces, become a part of the system control loop (e.g., medical and industrial systems). These terminals are typically embedded, single-purpose devices with restricted functionality, sometimes air-gapped and increasingly hardened. We describe a new way of attacking such terminals in which an adversary has only temporary, non-invasive, physical access to the terminal. In this attack, the adversary attaches a small device to the interface that connects user input peripherals to the terminal. The device executes the attack when the authorized user is performing safety-critical operations, by modifying or blocking user input, or injecting new input events. Given that the attacker has access to user input, the execution of this attack might seem trivial. However, to succeed, the attacker needs to overcome a number of challenges including the inability to directly observe the user interface and avoid being detected by the users. We present techniques that allow user interface state and input tracking. We evaluate these techniques and show that they can be implemented efficiently. We further evaluate the effectiveness of our attack through an online user study and find input modification attacks that are hard for the users to detect and would therefore lead to serious violations of the input integrity.

==> intro-first.tex <==

\section{Introduction}
\label{sec:intro}

Many safety-critical systems reside in locations that untrusted people can temporarily access. In hospitals, medical devices are often kept in rooms that visitors may enter. In industrial facilities, the cleaning personnel can routinely access safety-critical systems, such as process control devices. In traffic control centers, the maintenance personnel may gain brief and unattended access to traffic signaling terminals.

Once the adversary has gained temporary physical access to a safety-critical system, he can try to attack it in different ways. In a straight-forward attack, the adversary enters a hospital room  where a safety-critical medical device is kept and changes its settings through user interface. Many medical devices do not require user authentication (e.g., password entry) as doctors must be able to operate them without interruptions. Such an attack is quick to perform, but the applied changes remain visible on the user interface of the target system. The doctor is likely to notice any pre-configured, dangerous settings when using the medical device for the next time.

In a more sophisticated attack, the adversary installs malicious software on the medical device and the malware modifies the device settings when the doctor is using the device. If the changes are performed at a carefully chosen moment, the doctor has little time to notice the attack before confirming the safety-critical operation. Installing malware on the target device may require a more invasive operation (e.g., opening the device enclosure) which is not always possible. Additionally, the installed malicious software is visible to a malware scan, as the legitimate software configuration of the safety-critical system is typically known and certified.

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/sketch}
  \caption{Attack scenario overview. A small attack device is attached to the target device USB port and it performs the attack by observing and injecting user input events.}
  \label{fig:sketch}
\end{figure}

In this paper we describe a novel attack that is quick to deploy on the target location, difficult to notice for the user, and impossible to catch using typical malware detection. We call the attack \emph{hacking in the blind}. In the attack, the adversary gains physical access to a safety-critical system, attaches a small attack device to its USB port, and leaves the location (see Figure~\ref{fig:sketch}). The attached device observes communication between a user interaction peripheral, such as a mouse, and the target system. When the legitimate user is performing a safety-critical operation (e.g., the doctor modifies the medical device settings), the attached device launches the attack by injecting new user input events to the target system. On the safety-critical systems we consider, the attack can result in serious safety violation, even loss of a human life.

The attack requires only brief and non-invasive access to the target device---attaching a small USB device takes a few seconds. A small device can be difficult to notice on casual inspection and the adversary can collect the device back, once the attack has been successfully performed. To a malware detection system the attack is completely invisible, as no malicious code is running on the target system. The only chance to detect the attack is that the legitimate user notices the subtle visual changes on the UI when the attack is active (e.g., medical device settings are modified). Previous studies have shown that people often do not notice minor visual change \cite{simons2005}. 

Realization of our attacks involves also technical challenges. As the attack device only sees the incoming user input events, its view of the target system is very limited. We explore attacks that can be launched based on partial knowledge of the target system state, develop a novel state tracking algorithm, and design attack launch techniques that give little visual indication to the user. Because our attack is invisible to traditional malware detection, it operates under a limited view of the target system, and gives little indication to the user, we call it hacking in the blind.

We evaluated the attack using a user interface of a pacemaker programmer as a case study. Our evaluation on \red{x} online study participants shows that our algorithm can efficiently determine the current state of the target system. We tested different attack variants on \red{x} participants and noticed that such attacks can be indeed difficult to notice. Only \red{x\%} reported any suspicious activity in the user interface during an attack. We conclude that our attacks presents a serious threat to many current safety-critical systems.

To summarize, in this paper we make the following contributions: 

\begin{packed_itemize}
	\item \textbf{Novel attack approach.} We present a new way to attack safety-critical systems. The attack is quick to deploy, hard for users to notice, and completely invisible to malware detection.

	\item \textbf{State tracking algorithm.} We developed novel state estimation techniques, including an algorithm that estimates the most likely state of the target system based on the observed user inputs. 

%    \item \textbf{User study results.} We evaluate our attacks on \red{x} online study participants. These initial study results demonstrate that our attacks can be hard to notice.
	\item \textbf{UI manipulation techniques.} Using an online user study, we evaluated attack launch mechanisms that require limited knowledge of the system state and provide little visual indication to the user. 

    \item \textbf{Protective measures.} We discus user interface design techniques for safety-critical systems that can help to protect against our attacks.
\end{packed_itemize}

The rest of the paper is organized as follows. In Section~\ref{sec:scenario} we explain the attack scenario and assumptions. We describe our attack approach and techniques in Section~\ref{sec:overview}. We present our user study results in Section~\ref{sec:evaluation}. In Section~\ref{sec:analysis} we analyze attack detection and prevention. We discuss attack deployment and future work in Section~\ref{sec:discussion}. Section~\ref{sec:related} reviews related work and we conclude in Section~\ref{sec:conclusion}.


